A comprehensive approach to dark matter studies: exploration of simplified top-philic models

Studies of dark matter lie at the interface of collider physics, astrophysics and cosmology. Constraining models featuring dark matter candidates entails the capability to provide accurate predictions for large sets of observables and compare them to a wide spectrum of data. We present a framework which, starting from a model lagrangian, allows one to consistently and systematically make predictions, as well as to confront those predictions with a multitude of experimental results. As an application, we consider a class of simplified dark matter models where a scalar mediator couples only to the top quark and a fermionic dark sector (i.e. the simplified top-philic dark matter model). We study in detail the complementarity of relic density, direct/indirect detection and collider searches in constraining the multi-dimensional model parameter space, and efficiently identify regions where individual approaches to dark matter detection provide the most stringent bounds. In the context of collider studies of dark matter, we point out the complementarity of LHC searches in probing different regions of the model parameter space with final states involving top quarks, photons, jets and/or missing energy. Our study of dark matter production at the LHC goes beyond the tree-level approximation and we show examples of how higher-order corrections to dark matter production processes can affect the interpretation of the experimental results.

==> table_ref.tex <==
\begin{table}
\center
\begin{tabular}{l|p{1.30cm}clp{5.5cm}}
  & &  \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/id_tt}} & $\mdm>m_t$ &  \\
  Cosmology &relic$\qquad~$ indirect& \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/id_aa}} & $\mdm<m_t$ & Planck~\cite{Planck:2015xua}, FermiLAT~\cite{Ackermann:2015zua,Ackermann:2015lka}\\
  Astrophysics && \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/id_yy} } & $\mdm>\my$ & \\[5mm]
\cline{2-5}\\[-2mm]
 & direct & \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/dd}} & $\mdm>1$~GeV & LUX~\cite{Akerib:2013tjd}, CDMSLite~\cite{Agnese:2015nto} \\[5mm]
\hline \\[-2mm]
 \multirow{5}{*}{Colliders}
 & \multirow{2}{*}{$\MET$}
  &  \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/met_tt}} & $\my>2\mdm$ & $+ t\bar t$~\cite{Aad:2014vea,Khachatryan:2015nua} \\ 
  && \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/met_a}} & $\my>2\mdm$ & $+ j$~\cite{Aad:2015zva,Khachatryan:2014rra,CMS:2015jdt},
       $+ Z$~\cite{Aad:2013oja,Aad:2014vka,CMS:2015jha,Khachatryan:2015bbl,ATLAS:monoZ}, $+ h$~\cite{Aad:2015dva,Aad:2015yga,monoh1,monoh2} \\[2mm]
\cline{2-5}\\[-2mm]
 & \multirow{3}{*}{no $\MET$}
  &   \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/nonmet_tttt}}
  & $\my>2m_t$ & 4$t$~\cite{Chatrchyan:2013fea,Khachatryan:2014sca} \\
  &&  \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/nonmet_tt}}
  & $\my>2m_t$ & $t\bar t$~\cite{Aad:2015fna,Khachatryan:2015sma} \\
  &&  \raisebox{-.4\height}{\includegraphics[height=1cm]{diagrams/nonmet_aa}}
  & $\my<2m_t$ & $jj$~\cite{Aad:2014aqa,ATLAS:2015nsi,CMS:2015neg,Khachatryan:2015dcf}, $\gamma\gamma$~\cite{atlasDigamma,CMS:2015dxe, Aad:2015mna, Khachatryan:2015qba} \\
\end{tabular}
\caption{Signatures of our simplified top-philic DM model. 
 }
\label{tab:sig}
\end{table}

